AGMixup: Adaptive Graph Mixup for Semi-supervised Node Classification

Mixup is a data augmentation technique that enhances model generalization by interpolating between data points using a mixing ratio $\lambda$ in the image domain. Recently, the concept of mixup has been adapted to the graph domain through node-centric interpolations. However, these approaches often fail to address the complexity of interconnected relationships, potentially damaging the graph's natural topology and undermining node interactions. Furthermore, current graph mixup methods employ a one-size-fits-all strategy with a randomly sampled $\lambda$ for all mixup pairs, ignoring the diverse needs of different pairs. This paper proposes an Adaptive Graph Mixup (AGMixup) framework for semi-supervised node classification. AGMixup introduces a subgraph-centric approach, which treats each subgraph similarly to how images are handled in Euclidean domains, thus facilitating a more natural integration of mixup into graph-based learning. We also propose an adaptive mechanism to tune the mixing ratio $\lambda$ for diverse mixup pairs, guided by the contextual similarity and uncertainty of the involved subgraphs. Extensive experiments across seven datasets on semi-supervised node classification benchmarks demonstrate AGMixup's superiority over state-of-the-art graph mixup methods. Source codes are available at \url{https://github.com/WeigangLu/AGMixup}.

==> tables/semi.tex <==
\begin{table*}[ht!]
    \centering
    
%    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{l c c c c c c  c}
    \hline
    \toprule
%    ~ & \multicolumn{3}{c}{\textbf{Medium Graphs}} & \multicolumn{3}{c}{\textbf{Large Graphs}} & \multirow{4}{*}{\textbf{Avg. Gains}} \\
    
    ~ & \textbf{Cora} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{CS} & \textbf{Physics} & \textbf{Arxiv} & ~ \\
%    \midrule
	\cmidrule(r){2-7}  
	
	\textbf{\# Nodes} & \emph{2.7k} & \emph{3.3k} & \emph{19.7k} & \emph{18.3k} & \emph{34.4k} & \emph{169.3k} & ~\\
	\textbf{\# Edges} & \emph{5.2k} & \emph{4.6k} & \emph{44.3k} & \emph{81.8k} & \emph{247.9k}2 & \emph{1166.2k} & \textbf{Avg. Gains}\\

%	\cmidrule(r){1-1} \cmidrule(r){2-7} \cmidrule(r){8-8} 
	\midrule
	GCN  
    & 80.51$_{\pm1.39}$ 
    & 69.53$_{\pm0.96}$ 
    & 78.23$_{\pm1.64}$ 
    & 91.22$_{\pm0.83}$ 
    & 93.51$_{\pm0.34}$ 
    & 65.39$_{\pm0.13}$ 
    & \zero \\
    \hdashline[5pt/4pt]
    ~ + GraphMix 
    & 81.18$_{\pm1.03}$ 
    & 69.67$_{\pm0.96}$ 
    & 78.07$_{\pm1.99}$ 
    & 91.27$_{\pm0.97}$ 
    & 93.54$_{\pm0.73}$ 
    & 65.27$_{\pm0.29}$ 
    & \imp{0.12} \\
    
    ~ + NodeMixup 
    & 81.21$_{\pm1.02}$ 
    & 69.45$_{\pm0.74}$ 
    & 78.98$_{\pm1.32}$ 
    & 92.03$_{\pm0.36}$ 
    & 93.86$_{\pm0.67}$ 
    & 66.82$_{\pm0.24}$ 
    & \imp{0.86}\\
    
    ~ + iGraphMix 
    & 81.16$_{\pm0.95}$ 
    & 69.95$_{\pm0.84}$ 
    & 77.07$_{\pm1.61}$ 
    & 90.93$_{\pm0.68}$ 
    & 93.61$_{\pm0.36}$ 
    & 65.97$_{\pm0.57}$ 
    & \imp{0.10}\\
    
    ~ + \textbf{\agmixup (\textit{ours})}
    & \textbf{83.61}$_{\pm0.39}$ & \textbf{70.63}$_{\pm1.54}$ & \textbf{81.90}$_{\pm0.40}$ & \textbf{92.35}$_{\pm0.92}$ & \textbf{94.45}$_{\pm0.42}$ & \textbf{67.96}$_{\pm0.21}$ & \imp{\textbf{2.71}}\\ 
    
    \midrule
%	\cmidrule(r){1-1} \cmidrule(r){2-4}  \cmidrule(r){5-7} \cmidrule(r){8-8}
	    
    GAT 
    & 80.02$_{\pm1.15}$ 
    & 68.38$_{\pm1.35}$ 
    & 77.28$_{\pm1.80}$ 
    & 90.06$_{\pm0.80}$ 
    & 92.59$_{\pm0.64}$ 
    & 66.57$_{\pm0.27}$ & 
    \zero\\
    \hdashline[5pt/4pt]
    ~ + GraphMix 
    & 80.07$_{\pm1.11}$ 
    & 69.53$_{\pm0.76}$ 
    & 76.96$_{\pm1.85}$ 
    & 88.43$_{\pm1.49}$ 
    & 91.73$_{\pm1.47}$ 
    & 65.84$_{\pm0.18}$ 
    & \dec{0.41}\\
    
    ~ + NodeMixup 
    & 81.46$_{\pm1.13}$ 
    & 69.21$_{\pm0.86}$ 
    & 78.03$_{\pm1.03}$ 
    & 90.86$_{\pm1.23}$ 
    & 92.84$_{\pm1.42}$ 
    & 66.72$_{\pm0.26}$ 
    & \imp{0.89}\\
    
    ~ + iGraphMix 
    & 80.07$_{\pm1.20}$ 
    & 69.11$_{\pm0.79}$ 
    &77.14$_{\pm1.35}$ 
    & 90.01$_{\pm0.99}$ 
    & 92.64$_{\pm0.69}$ 
    & 64.79$_{\pm0.51}$ 
    & \dec{0.28}\\
    
    ~ + \textbf{\agmixup (\textit{ours})}
    & \textbf{83.14}$_{\pm0.54}$ & \textbf{69.72}$_{\pm1.51}$ & \textbf{81.60}$_{\pm0.51}$ & \textbf{91.92}$_{\pm1.41}$ & \textbf{94.31}$_{\pm0.63}$  & \textbf{67.48}$_{\pm0.72}$ & \imp{\textbf{2.78}}\\ 

    \midrule
%	\cmidrule(r){1-1} \cmidrule(r){2-4}  \cmidrule(r){5-7} \cmidrule(r){8-8}
	    
    JKNet 
    & 79.48$_{\pm1.47}$ 
    & 67.45$_{\pm1.05}$ 
    & 77.52$_{\pm2.29}$ 
    & 89.93$_{\pm1.11}$ 
    & 92.59$_{\pm1.36}$ 
    & 67.39$_{\pm0.18}$ 
    & \zero\\
     \hdashline[5pt/4pt]
    ~ + GraphMix 
    & 80.14$_{\pm1.29}$ 
    & 67.75$_{\pm1.01}$ 
    & 78.11$_{\pm2.12}$ 
    & 90.97$_{\pm0.85}$ 
    & 92.68$_{\pm1.09}$ 
    & 66.59$_{\pm0.13}$ 
    & \imp{0.35}\\
    
    ~ + NodeMixup 
    & 80.94$_{\pm1.03}$ 
    & \textbf{68.08}$_{\pm1.41}$ 
    & 78.96$_{\pm1.61}$ 
    & 91.71$_{\pm0.98}$ 
    & 92.44$_{\pm1.24}$ &
     67.98$_{\pm0.42}$ 
    & \imp{1.22}\\
    
    ~ + iGraphMix 
    & 79.94$_{\pm1.03}$ 
    & 67.58$_{\pm0.99}$ 
    & 76.03$_{\pm2.10}$ 
    & 91.19$_{\pm0.58}$ 
    & 92.83$_{\pm0.86}$ 
    & 65.15$_{\pm0.81}$ 
    & \dec{0.46}\\
    
    ~ + \textbf{\agmixup (\textit{ours})} 
    & \textbf{82.06}$_{\pm0.83}$ & 68.00$_{\pm1.53}$ & \textbf{81.34}$_{\pm0.44}$  & \textbf{92.63}$_{\pm0.50}$ & \textbf{93.27}$_{\pm0.62}$ & \textbf{69.76}$_{\pm0.21}$ & \imp{\textbf{2.70}}\\ 
    
   
    \midrule
%	\cmidrule(r){1-1} \cmidrule(r){2-4}  \cmidrule(r){5-7} \cmidrule(r){8-8}
	    
    GraphSAGE 
    & 79.28$_{\pm1.20}$ 
    & 68.36$_{\pm0.89}$ 
    & 75.72$_{\pm1.84}$ 
    & 91.95$_{\pm0.36}$ 
    & 93.18$_{\pm0.47}$ 
    & 66.00$_{\pm0.17}$ 
    & \zero\\
    \hdashline[5pt/4pt]
    ~ + GraphMix 
    & 79.65$_{\pm1.44}$ 
    & 68.44$_{\pm1.21}$ 
    & 75.88$_{\pm1.89}$ 
    & 91.71$_{\pm0.52}$ 
    & 92.93$_{\pm0.59}$ 
    & 66.73$_{\pm0.14}$ 
    & \imp{0.22}\\

    ~ + NodeMixup 
    & 80.42$_{\pm1.23}$ 
    & 69.06$_{\pm0.58}$ 
    & 77.92$_{\pm1.72}$ 
    & 91.94$_{\pm0.38}$ 
    & 93.78$_{\pm0.68}$ 
    & 67.13$_{\pm0.21}$ 
    & \imp{1.28}\\
    
    ~ + iGraphMix 
    & 79.72$_{\pm1.14}$ 
    & 68.30$_{\pm0.82}$ 
    & 75.70$_{\pm1.67}$ 
    & 91.70$_{\pm0.61}$ 
    & 92.80$_{\pm0.77}$ 
    & 64.66$_{\pm0.47}$ 
    & \dec{0.37}\\
    ~ + \textbf{\agmixup (\textit{ours})} 
    & \textbf{82.67}$_{\pm1.16}$ & \textbf{70.04}$_{\pm1.08}$ & \textbf{79.84}$_{\pm0.74}$  & \textbf{92.31}$_{\pm0.50}$ & \textbf{94.28}$_{\pm0.64}$  & \textbf{68.82}$_{\pm0.11}$ & \imp{\textbf{3.00}}\\ 
    
    \bottomrule
	\addlinespace
    \multicolumn{8}{l}{\footnotesize{The best accuracy is marked in \textbf{bold} according to each backbone model. Results on ogbn-products are in the Appendix.}}
    \end{tabular}
%    }
    \caption{Semi-supervised Node Classification Results (\%).\label{tab:semi}}

\end{table*}


%\begin{table}[ht!]
%    \centering
%    \caption{Semi-supervised Node Classification Results across Six Graphs.}
%    \resizebox{0.9\linewidth}{!}{
%    \begin{tabular}{l c c c c c c  c}
%    \hline
%    \toprule
%    ~ & \multicolumn{3}{c}{\textbf{Medium Graphs}} & \multicolumn{3}{c}{\textbf{Large Graphs}} & \multirow{4}{*}{\textbf{Avg. Gains}} \\
%    
%    ~ & Cora & Citeseer & Pubmed & CS & Physics & Arxiv & ~ \\
%%    \midrule
%	\cmidrule(r){2-4}  \cmidrule(r){5-7} 
%	\textbf{\# Nodes} & \emph{2.7k} & \emph{3.3k} & \emph{19.7k} & \emph{18.3k} & \emph{34.4k} & \emph{169.3k} & ~\\
%	\textbf{\# Edges} & \emph{5.2k} & \emph{4.6k} & \emph{44.3k} & \emph{81.8k} & \emph{247.9k} & \emph{1166.2k} & ~\\
%
%	\midrule
%	GCN  
%    & \cellcolor[HTML]{FDECEE}80.51$_{\pm1.39}$ 
%    & 69.53$_{\pm0.96}$ 
%    & \cellcolor[HTML]{FDECEE}78.23$_{\pm1.64}$ 
%    & \cellcolor[HTML]{FDECEE}91.22$_{\pm0.83}$ 
%    & \cellcolor[HTML]{FDECEE}93.51$_{\pm0.34}$ 
%    & \cellcolor[HTML]{FDECEE}65.39$_{\pm0.13}$ 
%    & \zero \\
%    
%    ~ + GraphMix 
%    & \cellcolor[HTML]{FDECEE}81.18$_{\pm1.03}$ 
%    & 69.67$_{\pm0.96}$ 
%    & \cellcolor[HTML]{FDECEE}78.07$_{\pm1.99}$ 
%    & \cellcolor[HTML]{FDECEE}91.27$_{\pm0.97}$ 
%    & \cellcolor[HTML]{FDECEE}93.54$_{\pm0.73}$ 
%    & \cellcolor[HTML]{FDECEE}65.27$_{\pm0.29}$ 
%    & \imp{0.12} \\
%    
%    ~ + NodeMixup 
%    & \cellcolor[HTML]{FDECEE}81.21$_{\pm1.02}$ 
%    & \cellcolor[HTML]{FDECEE}69.45$_{\pm0.74}$ 
%    & \cellcolor[HTML]{FDECEE}78.98$_{\pm1.32}$ 
%    & 92.03$_{\pm0.36}$ 
%    & \cellcolor[HTML]{FDECEE}93.86$_{\pm0.67}$ 
%    & \cellcolor[HTML]{FDECEE}66.82$_{\pm0.24}$ 
%    & \imp{0.86}\\
%    
%    ~ + iGraphMix 
%    & \cellcolor[HTML]{FDECEE}81.16$_{\pm0.95}$ 
%    & 69.95$_{\pm0.84}$ 
%    & \cellcolor[HTML]{FDECEE}77.07$_{\pm1.61}$ 
%    & \cellcolor[HTML]{FDECEE}90.93$_{\pm0.68}$ 
%    & \cellcolor[HTML]{FDECEE}93.61$_{\pm0.36}$ 
%    & \cellcolor[HTML]{FDECEE}65.97$_{\pm0.57}$ 
%    & \imp{0.10}\\
%    
%    ~ + \textbf{\agmixup (\textit{ours})}
%    & \textbf{83.61}$_{\pm0.39}$ & \textbf{70.63}$_{\pm1.54}$ & \textbf{81.90}$_{\pm0.40}$ & \textbf{92.35}$_{\pm0.92}$ & \textbf{94.45}$_{\pm0.42}$ & \textbf{67.96}$_{\pm0.21}$ & \imp{2.71}\\ 
%    
%%    \midrule
%	\cmidrule(r){1-1} \cmidrule(r){2-4}  \cmidrule(r){5-7} \cmidrule(r){8-8}
%	    
%    GAT 
%    & \cellcolor[HTML]{FDECEE}80.02$_{\pm1.15}$ 
%    & 68.38$_{\pm1.35}$ 
%    & \cellcolor[HTML]{FDECEE}77.28$_{\pm1.80}$ 
%    & \cellcolor[HTML]{FDECEE}90.06$_{\pm0.80}$ 
%    & \cellcolor[HTML]{FDECEE}92.59$_{\pm0.64}$ 
%    & \cellcolor[HTML]{FDECEE}66.57$_{\pm0.27}$ & 
%    \zero\\
%    
%    ~ + GraphMix 
%    & \cellcolor[HTML]{FDECEE}80.07$_{\pm1.11}$ 
%    & 69.53$_{\pm0.76}$ 
%    & \cellcolor[HTML]{FDECEE}76.96$_{\pm1.85}$ 
%    & \cellcolor[HTML]{FDECEE}88.43$_{\pm1.49}$ 
%    & \cellcolor[HTML]{FDECEE}91.73$_{\pm1.47}$ 
%    & \cellcolor[HTML]{FDECEE}65.84$_{\pm0.18}$ 
%    & \dec{0.41}\\
%    
%    ~ + NodeMixup 
%    & \cellcolor[HTML]{FDECEE}81.46$_{\pm1.13}$ 
%    & 69.21$_{\pm0.86}$ 
%    & \cellcolor[HTML]{FDECEE}78.03$_{\pm1.03}$ 
%    & 90.86$_{\pm1.23}$ 
%    & \cellcolor[HTML]{FDECEE}92.84$_{\pm1.42}$ 
%    & \cellcolor[HTML]{FDECEE}66.72$_{\pm0.26}$ 
%    & \imp{0.89}\\
%    
%    ~ + iGraphMix 
%    & \cellcolor[HTML]{FDECEE}80.07$_{\pm1.20}$ 
%    & 69.11$_{\pm0.79}$ 
%    &\cellcolor[HTML]{FDECEE}77.14$_{\pm1.35}$ 
%    & \cellcolor[HTML]{FDECEE}90.01$_{\pm0.99}$ 
%    & \cellcolor[HTML]{FDECEE}92.64$_{\pm0.69}$ 
%    & \cellcolor[HTML]{FDECEE}64.79$_{\pm0.51}$ 
%    & \dec{0.28}\\
%    
%    ~ + \textbf{\agmixup (\textit{ours})}
%    & \textbf{83.14}$_{\pm0.54}$ & \textbf{69.72}$_{\pm1.51}$ & \textbf{81.60}$_{\pm0.51}$ & \textbf{91.92}$_{\pm1.41}$ & \textbf{94.31}$_{\pm0.63}$  & \textbf{67.48}$_{\pm0.72}$ & \imp{2.78}\\ 
%    
%%    \midrule
%	\cmidrule(r){1-1} \cmidrule(r){2-4}  \cmidrule(r){5-7} \cmidrule(r){8-8}
%	    
%    JKNet 
%    & \cellcolor[HTML]{FDECEE}79.48$_{\pm1.47}$ 
%    & 67.45$_{\pm1.05}$ 
%    & \cellcolor[HTML]{FDECEE}77.52$_{\pm2.29}$ 
%    & \cellcolor[HTML]{FDECEE}89.93$_{\pm1.11}$ 
%    & \cellcolor[HTML]{FDECEE}92.59$_{\pm1.36}$ 
%    & \cellcolor[HTML]{FDECEE}67.39$_{\pm0.18}$ 
%    & \zero\\
%    
%    ~ + GraphMix 
%    & \cellcolor[HTML]{FDECEE}80.14$_{\pm1.29}$ 
%    & 67.75$_{\pm1.01}$ 
%    & \cellcolor[HTML]{FDECEE}78.11$_{\pm2.12}$ 
%    & \cellcolor[HTML]{FDECEE}90.97$_{\pm0.85}$ 
%    & 92.68$_{\pm1.09}$ 
%    & \cellcolor[HTML]{FDECEE}66.59$_{\pm0.13}$ 
%    & \imp{0.35}\\
%    
%    ~ + NodeMixup 
%    & \cellcolor[HTML]{FDECEE}80.94$_{\pm1.03}$ 
%    & \textbf{68.08}$_{\pm1.41}$ 
%    & \cellcolor[HTML]{FDECEE}78.96$_{\pm1.61}$ 
%    & \cellcolor[HTML]{FDECEE}91.71$_{\pm0.98}$ 
%    & 92.44$_{\pm1.24}$ &
%     \cellcolor[HTML]{FDECEE}67.98$_{\pm0.42}$ 
%    & \imp{1.22}\\
%    
%    ~ + iGraphMix 
%    & \cellcolor[HTML]{FDECEE}79.94$_{\pm1.03}$ 
%    & 67.58$_{\pm0.99}$ 
%    & \cellcolor[HTML]{FDECEE}76.03$_{\pm2.10}$ 
%    & \cellcolor[HTML]{FDECEE}91.19$_{\pm0.58}$ 
%    & 92.83$_{\pm0.86}$ 
%    & \cellcolor[HTML]{FDECEE}65.15$_{\pm0.81}$ 
%    & \dec{0.46}\\
%    
%    ~ + \textbf{\agmixup (\textit{ours})} 
%    & \textbf{82.06}$_{\pm0.83}$ & 68.00$_{\pm1.53}$ & \textbf{81.34}$_{\pm0.44}$  & \textbf{92.63}$_{\pm0.50}$ & \textbf{93.27}$_{\pm0.62}$ & \textbf{69.76}$_{\pm0.21}$ & \imp{2.70}\\ 
%    
%%    \midrule
%	\cmidrule(r){1-1} \cmidrule(r){2-4}  \cmidrule(r){5-7} \cmidrule(r){8-8}
%	    
%    GraphSAGE 
%    & \cellcolor[HTML]{FDECEE}79.28$_{\pm1.20}$ 
%    & \cellcolor[HTML]{FDECEE}68.36$_{\pm0.89}$ 
%    & \cellcolor[HTML]{FDECEE}75.72$_{\pm1.84}$ 
%    & 91.95$_{\pm0.36}$ 
%    & \cellcolor[HTML]{FDECEE}93.18$_{\pm0.47}$ 
%    & \cellcolor[HTML]{FDECEE}66.00$_{\pm0.17}$ 
%    & \zero\\
%    
%    ~ + GraphMix 
%    & \cellcolor[HTML]{FDECEE}79.65$_{\pm1.44}$ 
%    & \cellcolor[HTML]{FDECEE}68.44$_{\pm1.21}$ 
%    & \cellcolor[HTML]{FDECEE}75.88$_{\pm1.89}$ 
%    & \cellcolor[HTML]{FDECEE}91.71$_{\pm0.52}$ 
%    & \cellcolor[HTML]{FDECEE}92.93$_{\pm0.59}$ 
%    & \cellcolor[HTML]{FDECEE}66.73$_{\pm0.14}$ 
%    & \imp{0.22}\\
%
%    ~ + NodeMixup 
%    & \cellcolor[HTML]{FDECEE}80.42$_{\pm1.23}$ 
%    & \cellcolor[HTML]{FDECEE}69.06$_{\pm0.58}$ 
%    & \cellcolor[HTML]{FDECEE}77.92$_{\pm1.72}$ 
%    & 91.94$_{\pm0.38}$ 
%    & 93.78$_{\pm0.68}$ 
%    & \cellcolor[HTML]{FDECEE}67.13$_{\pm0.21}$ 
%    & \imp{1.28}\\
%    
%    ~ + iGraphMix 
%    & \cellcolor[HTML]{FDECEE}79.72$_{\pm1.14}$ 
%    & \cellcolor[HTML]{FDECEE}68.30$_{\pm0.82}$ 
%    & \cellcolor[HTML]{FDECEE}75.70$_{\pm1.67}$ 
%    & \cellcolor[HTML]{FDECEE}91.70$_{\pm0.61}$ 
%    & \cellcolor[HTML]{FDECEE}92.80$_{\pm0.77}$ 
%    & \cellcolor[HTML]{FDECEE}64.66$_{\pm0.47}$ 
%    & \dec{0.37}\\
%    ~ + \textbf{\agmixup (\textit{ours})} 
%    & \textbf{82.67}$_{\pm1.16}$ & \textbf{70.04}$_{\pm1.08}$ & \textbf{79.84}$_{\pm0.74}$  & \textbf{92.31}$_{\pm0.50}$ & \textbf{94.28}$_{\pm0.64}$  & \textbf{68.82}$_{\pm0.11}$ & \imp{3.00}\\ 
%    
%    \bottomrule
%	\addlinespace
%    \multicolumn{8}{l}{\footnotesize{The best accuracy is marked in \textbf{bold} according to each backbone model.}}
%    
%	\label{tab:semi}
%    \end{tabular}
%    }
%    
%\end{table}

